DreamCar: Leveraging Car-specific Prior for in-the-wild 3D Car Reconstruction

Self-driving industries usually employ professional artists to build exquisite 3D cars. However, it is expensive to craft large-scale digital assets. Since there are already numerous datasets available that contain a vast number of images of cars, we focus on reconstructing high-quality 3D car models from these datasets. However, these datasets only contain one side of cars in the forward-moving scene. We try to use the existing generative models to provide more supervision information, but they struggle to generalize well in cars since they are trained on synthetic datasets not car-specific. In addition, The reconstructed 3D car texture misaligns due to a large error in camera pose estimation when dealing with in-the-wild images. These restrictions make it challenging for previous methods to reconstruct complete 3D cars. To address these problems, we propose a novel method, named DreamCar, which can reconstruct high-quality 3D cars given a few images even a single image. To generalize the generative model, we collect a car dataset, named Car360, with over 5,600 vehicles. With this dataset, we make the generative model more robust to cars. We use this generative prior specific to the car to guide its reconstruction via Score Distillation Sampling. To further complement the supervision information, we utilize the geometric and appearance symmetry of cars. Finally, we propose a pose optimization method that rectifies poses to tackle texture misalignment. Extensive experiments demonstrate that our method significantly outperforms existing methods in reconstructing high-quality 3D cars. \href{https://xiaobiaodu.github.io/dreamcar-project/}{Our code is available.}

==> sec/3drec.tex <==


\section{3D Reconstruction}
As shown in \cref{vis_3drec}, we show additional 3D reconstruction results in the testing set of our Car360-Real dataset. This visualization highlights how current state-of-the-art methods face difficulties in achieving a realistic and complete 3D car model with limited supervision. Conversely, our approach effectively achieves a complete geometric reconstruction and detailed texture by leveraging the proposed mirror symmetry and car-specific priors.


\begin{figure}[t] % 'h' specifies here placement (here) of the figure
    \centering
    \includegraphics[width=0.8\textwidth]{figs/3drec.pdf} 
    \caption{\textbf{The additional comparison of different reconstruction methods in the testing set of Car360-Real.}}
    \label{vis_3drec}
    \vspace{-3mm}
\end{figure}

\begin{figure}[t] % 'h' specifies here placement (here) of the figure
    \centering
    \includegraphics[width=0.8\textwidth]{figs/simu.pdf} 
    \caption{\textbf{Car simulation in the original Nuscenes scenes.} The red circle indicates the simulated car.}
    \label{vis_simu}
    \vspace{-5mm}
\end{figure}

==> sec/syn.tex <==


\section{Novel View Synthesis}
We compare our novel view synthesis results with those of the state-of-the-art methods. We randomly select 100 vehicles as the testing set from the collected Car360-Syn dataset. We confirm that there is no overlap between the training and testing set. As indicated in \cref{syn_test}, we show the quantitative metrics compared with different generative models. Zero-123-XL \cite{zero123} performs inferiorly than ours due to lack of the car-specific prior. Stable-Zero123 \cite{stable-zero123} limited by its training on a fixed camera radius, does not perform well on our testing set. SyncDreamer \cite{liu2023syncdreamer} also obtains poor results since it is trained on the fixed target elevation. Our method, leveraging the car-specific prior, outperforms these methods, as evidenced by both quantitative and qualitative results in \cref{vis_nvs}. 
Furthermore, our model, trained on the Car360 dataset, demonstrates superior generalization to real-world vehicles, unlike other models that struggle with generalization and produce unpleasant outputs.





\noindent\textbf{Necessity of Car360 Dataset.}   To demonstrate the importance of our Car360 dataset, we conduct additional visual comparisons on novel view synthesis. These comparisons show the improvement of Zero-123-XL by training it on our synthesized (Car360-Syn) and real-world (Car360-Real) datasets, progressively.  As shown in \cref{vis_car360}, our dataset significantly enhances the generalization of the model to real-world vehicles. Initially, Zero-123-XL struggles to generalize to real-world cars. However, with the incorporation of our dataset, we witness a substantial improvement in the generalization of models.














\begin{table}[t]
\centering
\scriptsize
\def\arraystretch{1.2}
\setlength{\tabcolsep}{6pt}
\caption{Evaluation in the test set of Car360-Syn Dataset}
\label{syn_test}
\begin{tabular}{c|ccc|c}
\toprule
     & Zero-123-XL \cite{zero123} & Stable-Zero123 \cite{stable-zero123} & SyncDreamer \cite{liu2023syncdreamer} & Ours            \\ \midrule \midrule
PSNR & 21.33      & 15.52          & 14.34       & \textbf{23.18  }         \\
SSIM & 0.8878     & 0.7952         & 0.7847      & \textbf{0.9043} \\
FID  & 0.82       & 2.21           & 2.48        & \textbf{0.016 }          \\ \bottomrule
\end{tabular}
\end{table}

\begin{figure}[t] % 'h' specifies here placement (here) of the figure
    \centering
    \includegraphics[width=0.8\textwidth]{figs/nvs.pdf} 
    \caption{\textbf{The additional comparison of novel view synthesis across 3D-aware diffusion models in the test set of Car360-Real.} Given input views in the first column, we use generative models to generate novel views to demonstrate which model can generate more stable and realistic results.}
    \label{vis_nvs}
    \vspace{-5mm}
\end{figure}


\begin{figure}[t] % 'h' specifies here placement (here) of the figure
    \centering
    \includegraphics[width=0.8\textwidth]{figs/adding_car.pdf} 
    \caption{\textbf{The additional comparison when Zero-123-XL trained on our collected Car360 dataset progressively.} }
    \label{vis_car360}
    \vspace{-5mm}
\end{figure}



